Quantifying the Impact of Biobanks and Cohort Studies

Biobanks advance biomedical and clinical research by collecting and offering data and biological samples for numerous studies. However, the impact of these repositories varies greatly due to differences in their purpose, scope, governance, and data collected. Here, we computationally identified 2,663 biobanks and their textual mentions in 228,761 scientific articles, 16,210 grants, 15,469 patents, 1,769 clinical trials, and 9,468 public policy documents, helping characterize the academic communities that utilize and support them. We found a strong concentration of biobank-related research on a few diseases, where 20\% of publications focus on obesity, Alzheimer's disease, breast cancer, and diabetes. Moreover, collaboration, rather than citation count, shapes the community's recognition of a biobank. We show that, on average, 41.1\% of articles miss to reference any of the biobank's reference papers and 59.6\% include a biobank member as a co-author. Using a generalized linear model, we identified the key factors that contribute to the impact of a biobank, finding that an impactful biobank tends to be more open to external researchers, and that quality data -- especially linked medical records -- as opposed to large data, correlates with a higher impact in science, innovation, and disease. The collected data and findings are accessible through an open-access web application intended to inform strategies to expand access and maximize the value of these valuable resources.

==> impact_snippets.tex <==
Scientific impact is a multifaceted concept that cannot be fully captured with a single variable. \rev{Conventional citation-based metrics often fail to capture the true value of scientific work, particularly in the case of biobanks, which lack standardized identifiers and therefore receive inadequate citation credit~\cite{cambon-thomsen_assessing_2003,bravo_developing_2015,mabile_quantifying_2013}. As a result, the multifaceted impact of biobanks remains largely invisible to citation counts~\cite{lawrence_barriers_2020,klingler_stakeholder_2022,vora_impacts_2015}, hence the importance of measuring their impact across other relevant dimensions including grant acquisition, innovation production, disease treatment, and public health. Moreover, biobank impact should consider factors that are often overlooked like their ability to form partnerships, foster collaboration, and create research capacity. To fill this metric gap, we analyzed metadata related to these factors across the 271,394 documents mentioning biobanks.}

% research impact
% research impact and funding: grant funding & publications, grant-based publications, clinical-trials-based publications, patent-based publications
The direct research impact of biobanks is measured by the 228,632 publications mentioning biobanks, together receiving 10.3 million citations. Additionally, 194,872 publications are indirectly impacted by biobank-related grants, patents, and clinical trials, from which 193,884 were funded with grants mentioning biobanks, and 988 cited a biobank-related clinical trial, resulting in a total of 423,504 impacted publications. Related to grant acquisition, researchers received \$30.8 billion USD in funding from 16,204 grants mentioning biobanks, with a median amount per grant of half a million dollars, showcasing the financial contribution of biobanks to research. Using the associated NIH activity code of each grant, we identified 1,359 grants meant for personnel training and 1,106 for institutional collaboration, indicating a substantial contribution to capacity building by biobank-related grants. Similarly, biobanks help boost the career of researchers through grant acquisition, as illustrated by the 393 biobank-related grants classified in an NIH research career program, a prestigious class of grants for career development, securing a total of \$349 million. 


% innovation: patents and clinical trials, and their citations
% disease treatment: therapeutic patents, clinical trials treatment, drugs, scope and depth of diseases
To assess biobanks' contribution to therapeutic innovation, we used the Cooperative Patent Classification (CPC) codes of 8,590 patents and the National Library of Medicine (NLM) classification of 1,765 trials mentioning a biobank. Among the analyzed patents, 5,189 focus on therapeutic applications, with a significant emphasis on chemotherapy development (2,360 patents), highlighting cancer treatment as a primary area of innovation. Similarly to patents, about half of the clinical trials test a therapeutic intervention (839 clinical trials), focusing on cardiovascular and metabolic diseases (515), followed by cancer treatments (138). While drug innovation is a common target of therapeutic applications, vaccines rarely are the aim, accounting to only 4\% and 2\% of patents and clinical trials, respectively. Relatively small biobanks like the Bandim Health Project with a population cohort based in Guinea-Bissau, stand out as valuable resources for their leadership in conducting vaccine trials for rare diseases (Figure~\ref{fig:top}A).

In terms of partnerships, the engagement of the private sector with biobanks is substantial in patents but less so in clinical trials and publications mentioning biobanks, with 36.1\% of patents being assigned to companies, but only present in 5.8\% of clinical trials and 3.8\% of publications. Within the private sector, the pharmaceutical industry is the main beneficiary of biobanks, with companies like Roche, Amgen, Johnson \& Johnson, Pfizer, MSD (Merck in the US and Canada), and AstraZeneca accounting for 17.9\% of all partnerships (1,761 in research papers, 790 in patents, and 21 in clinical trials). Contrastingly, no biobank-related grant is funded by the private sector, suggesting the partnership to be potentially imbalanced. In general, however, the great majority of biobank partnerships occur within the education sector, with Harvard University alone being part of 8.3\% of all the research and innovation documents. 


Public health is the primary focus of publications mentioning biobanks (39.5\%), surpassing clinical and basic science combined (24.7\% and 7.2\%, respectively). Policies, however, are the closest source of public health impact, as they are directly written by policymakers. Consequently, we examine 9,343 official policy documents mentioning a biobank published by 157 public organizations across 27 countries. Policy institutions impacted by biobanks are mainly found across national governmental agencies and international nonprofit organizations, the most frequent policy publishers being the US Government (4,388 policies), followed by the World Bank (520), the Government of the UK (487), the Urban Institute (468), and the World Health Organization (368). We observe that 29.4\% of all public health policies target either a social, clinic, or prevention factor of health, with different frequency orders for government (prevention, social, clinical) and nonprofit organizations (social, clinical, prevention), illustrating their distinct roles in biobank-related policies.
